Dreaming to Assist: Learning to Align with Human Objectives for Shared Control in High-Speed Racing

Tight coordination is required for effective human-robot teams in domains involving fast dynamics and tactical decisions, such as multi-car racing. In such settings, robot teammates must react to cues of a human teammate's tactical objective to assist in a way that is consistent with the objective (e.g., navigating left or right around an obstacle). To address this challenge, we present Dream2Assist, a framework that combines a rich world model able to infer human objectives and value functions, and an assistive agent that provides appropriate expert assistance to a given human teammate. Our approach builds on a recurrent state space model to explicitly infer human intents, enabling the assistive agent to select actions that align with the human and enabling a fluid teaming interaction. We demonstrate our approach in a high-speed racing domain with a population of synthetic human drivers pursuing mutually exclusive objectives, such as "stay-behind" and "overtake". We show that the combined human-robot team, when blending its actions with those of the human, outperforms the synthetic humans alone as well as several baseline assistance strategies, and that intent-conditioning enables adherence to human preferences during task execution, leading to improved performance while satisfying the human's objective.

==> table.tex <==

\begin{table*}[]
\centering
\scriptsize
\caption{Ablations. \todo{Need to finalize this}}
\label{tab:ablations}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|llllllll|llllllll}
\toprule
                                 & \multicolumn{8}{c|}{Pass / Stay}                                                                       & \multicolumn{8}{c}{Left / Right}                                                                       \\
                                 \cmidrule{2-17}
                                 & \multicolumn{4}{c|}{Hairpin}                                & \multicolumn{4}{c|}{Straightaway}      & \multicolumn{4}{c|}{Hairpin}                                & \multicolumn{4}{c}{Straightaway}       \\ 
                                        & Prog.            & Return         & Avg. Speed  & Coll. & Prog. & Return & Avg. Speed & Coll. & Prog. & Return & Avg. Speed & Coll. & Prog. & Return & Avg. Speed & Coll. \\ 
\midrule
% \multirow{2}{*}{\textsc{Dreamer}}      & -11.32\pm 13.58   & 0.45\pm 2.94  & 0.24\pm 0.16  & \multicolumn{1}{l|}{-0.09\pm 0.18} & -0.65\pm 4.57    & -0.06\pm 0.85 & -0.34\pm 0.28   & 0.01\pm 0.06  & 21.75\pm 28.67   & -1.99\pm 2.16  & 0.03\pm 1.29   & \multicolumn{1}{l|}{0.05 0.08}  & 10.84\pm 7.31    & -0.62\pm 0.32  & 6.22\pm 6.80   & -0.03\pm 0.11 \\
%                               & -21.08\pm 68.62   & 0.30\pm 0.43  & 2.72\pm 1.74  & \multicolumn{1}{l|}{0.03\pm 0.03}  & -6.12\pm 17.46   & -0.03\pm 0.09 & 0.26\pm 0.39    & 0.10\pm 0.15  & 10.04\pm 17.91   & -1.30\pm 1.75  & -0.02\pm 1.58  & \multicolumn{1}{l|}{-0.04\pm 0.08} & -1.06 6.20    & 0.16\pm 1.23   & -0.63\pm 1.83  & 0.01\pm 0.10  \\
% \multirow{2}{*}{\textsc{Dreamer-AIL}}  & -28.90\pm 46.15   & -5.69\pm 7.31 & 0.99\pm 0.15  & \multicolumn{1}{l|}{-0.30\pm 0.21} & -116.61\pm 58.66 & -9.73\pm 4.21 & -21.16\pm 10.59 & -0.36\pm 0.27 & -144.00\pm 89.86 & -7.09\pm 6.63  & -14.73\pm 9.39 & \multicolumn{1}{l|}{-0.36\pm 0.20} & -134.36\pm 13.02 & -2.52\pm 0.91  & -11.21\pm 7.58 & -0.50\pm 0.11 \\
%                               & -216.56\pm 145.63 & -1.72\pm 0.42 & 5.21\pm 2.32  & \multicolumn{1}{l|}{}  & -52.54\pm 45.90  & -1.59\pm 0.16 & -1.28\pm 1.19   & -0.09\pm 0.11 & -119.13\pm 79.87 & -4.48\pm 17.27 & -15.34\pm 5.59 & \multicolumn{1}{l|}{} & -126.28\pm 53.22 & -13.44\pm 7.03 & -23.47\pm 5.43 & -0.45\pm 0.24 \\
% \multirow{2}{*}{\textsc{Dream2Assist}} & 71.81\pm 43.94    & -1.21\pm 3.28 & 0.68\pm 0.08  & \multicolumn{1}{l|}{-0.15\pm 0.24} & 5.99\pm 9.13     & -0.35\pm 1.44 & -1.08\pm -4.70  & -0.05\pm 0.07 & 54.82\pm 60.40   & 1.42\pm 5.19   & -0.90\pm 5.70  & \multicolumn{1}{l|}{-0.01\pm 0.10} & 4.98\pm 4.98     & 0.13\pm 0.52   & 0.10\pm 1.52   & 0.04\pm 0.10  \\
%                               & 60.46\pm 49.68    & 0.78\pm 0.39  & 6.91\pm 2.26  & \multicolumn{1}{l|}{0.14\pm 0.10}  & 57.78\pm 36.42   & -0.07\pm 0.21 & 2.16\pm 1.10    & 0.07\pm 0.09  & 27.20\pm 23.07   & 2.23\pm 2.33   & -3.25\pm 4.84  & \multicolumn{1}{l|}{-0.16\pm 0.18} & -1.09\pm 31.91   & -2.77\pm 2.43  & -2.74\pm 4.64  & 0.17\pm 0.15
\multirow{2}{*}{Dreamer}      & -11.32\pm 13.58   & 0.45\pm 2.94  & 0.24\pm 0.16  & \multicolumn{1}{l|}{-0.09 0.18} & -0.65 4.57    & -0.06 0.85 & -0.34 0.28   & 0.01 0.06  & 21.75 28.67   & -1.99 2.16  & 0.03 1.29   & \multicolumn{1}{l|}{0.05 0.08}  & 10.84 7.31    & -0.62 0.32  & 6.22 6.80   & -0.03 0.11 \\
                              & -21.08\pm 68.62   & 0.30\pm 0.43  & 2.72\pm 1.74  & \multicolumn{1}{l|}{0.03 0.03}  & -6.12 17.46   & -0.03 0.09 & 0.26 0.39    & 0.10 0.15  & 10.04 17.91   & -1.30 1.75  & -0.02 1.58  & \multicolumn{1}{l|}{-0.04 0.08} & -1.06 6.20    & 0.16 1.23   & -0.63 1.83  & 0.01 0.10  \\
\multirow{2}{*}{Dreamer-AIL}  & -28.90\pm 46.15   & -5.69\pm 7.31 & 0.99\pm 0.15  & \multicolumn{1}{l|}{-0.30 0.21} & -116.61 58.66 & -9.73 4.21 & -21.16 10.59 & -0.36 0.27 & -144.00 89.86 & -7.09 6.63  & -14.73 9.39 & \multicolumn{1}{l|}{-0.36 0.20} & -134.36 13.02 & -2.52 0.91  & -11.21 7.58 & -0.50 0.11 \\
                              & -216.56\pm 145.63 & -1.72\pm 0.42 & 5.21\pm 2.32  & \multicolumn{1}{l|}{0.06 0.19}  & -52.54 45.90  & -1.59 0.16 & -1.28 1.19   & -0.09 0.11 & -119.13 79.87 & -4.48 17.27 & -15.34 5.59 & \multicolumn{1}{l|}{-0.39 0.29} & -126.28 53.22 & -13.44 7.03 & -23.47 5.43 & -0.45 0.24 \\
\multirow{2}{*}{Dream2Assist} & 71.81\pm 43.94    & -1.21\pm 3.28 & 0.68\pm 0.08  & \multicolumn{1}{l|}{-0.15 0.24} & 5.99 9.13     & -0.35 1.44 & -1.08 -4.70  & -0.05 0.07 & 54.82 60.40   & 1.42 5.19   & -0.90 5.70  & \multicolumn{1}{l|}{-0.01 0.10} & 4.98 4.98     & 0.13 0.52   & 0.10 1.52   & 0.04 0.10  \\
                              & 60.46\pm 49.68    & 0.78\pm 0.39  & 6.91\pm 2.26  & \multicolumn{1}{l|}{0.14 0.10}  & 57.78 36.42   & -0.07 0.21 & 2.16 1.10    & 0.07 0.09  & 27.20 23.07   & 2.23 2.33   & -3.25 4.84  & \multicolumn{1}{l|}{-0.16 0.18} & -1.09 31.91   & -2.77 2.43  & -2.74 4.64  & 0.17 0.15  \\
\bottomrule
\end{tabular}
}
\end{table*}

